Measurement of the form factors of the decay B^+\to\bar D^{*0}\ell^+\nu_\ell and determination of the CKM matrix element |V_{cb}|

We present a measurement of the Cabibbo-Kobayashi-Maskawa matrix element $|V_{cb}|$ times the form factor normalization $\mathcal{F}(1)$ using the decay $B^+\to\bar D^{*0}\ell^+\nu_\ell$. This measurement is performed together with a determination of the form factor parameters $\rho^2$, $R_1(1)$ and $R_2(1)$ which fully characterize this decay in the framework of Heavy Quark Effective Theory. This analysis is based on a data sample equivalent to 140 fb$^{-1}$ of Belle data collected near the $\Upsilon(4S)$ resonance. The preliminary results, based on about 27,000 reconstructed $B^+\to\bar D^{*0}\ell^+\nu_\ell$ decays, are $\rho^2=1.376\pm 0.074\pm 0.056$, $R_1(1)=1.620\pm 0.091\pm 0.092$, $R_2(1)=0.805\pm 0.064\pm 0.036$ and $\mathcal{F}(1)|V_{cb}|=35.0\pm 0.4\pm 2.2$. We find the $B^+\to\bar D^{*0}\ell^+\nu_\ell$ branching fraction to be $(4.84\pm 0.04\pm 0.56)%$. For all numbers quoted here, the first error is the statistical and the second is the systematic uncertainty. A direct, model-independent determination of the form factor shapes has also been carried out and shows good agreement with the HQET based form factor parametrization by Caprini {\it et al.}.

==> ackn.tex <==
\section*{Acknowledgments}

%----------- Long version, for most papers ----------- 
We thank the KEKB group for the excellent operation of the
accelerator, the KEK cryogenics group for the efficient
operation of the solenoid, and the KEK computer group and
the National Institute of Informatics for valuable computing
and SINET3 network support. We acknowledge support from
the Ministry of Education, Culture, Sports, Science, and
Technology of Japan and the Japan Society for the Promotion
of Science; the Australian Research Council and the
Australian Department of Education, Science and Training;
the National Natural Science Foundation of China under
contract No.~10575109 and 10775142; the Department of
Science and Technology of India; 
the BK21 program of the Ministry of Education of Korea, 
the CHEP SRC program and Basic Research program 
(grant No.~R01-2005-000-10089-0) of the Korea Science and
Engineering Foundation, and the Pure Basic Research Group 
program of the Korea Research Foundation; 
the Polish State Committee for Scientific Research; 
%-> remove for now: under contract No.~2P03B 01324; 
the Ministry of Education and Science of the Russian
Federation and the Russian Federal Agency for Atomic Energy;
the Slovenian Research Agency;  the Swiss
National Science Foundation; the National Science Council
and the Ministry of Education of Taiwan; and the U.S.\
Department of Energy.


==> tabBackgroundNormalization.tex <==
% Table generated by Excel2LaTeX from sheet 'Background fractions'
\begin{tabular}{l|@{\extracolsep{.2cm}}cccc}
\hline\hline
           & $K \pi, e$ & $K \pi, \mu$ & $K3\pi, e$ & $K3\pi, \mu$  \\
\hline
    Signal &     0.872  $\pm$     0.020  &     0.843  $\pm$     0.020  &     0.947  $\pm$     0.032  &     0.945  $\pm$     0.033  \\

Signal correlated &     1.549  $\pm$     0.365  &     1.819  $\pm$     0.379  &     1.684  \scriptsize{\it (fixed)}  &     1.684  \scriptsize{\it (fixed)}  \\

       D** &     0.083  $\pm$     0.107  &     0.082  $\pm$     0.110  &     0.083  \scriptsize{\it (fixed)}  &     0.083  \scriptsize{\it (fixed)}  \\

Uncorrelated &     0.842  $\pm$     0.091  &     0.878  $\pm$     0.090  &     1.211  $\pm$     0.140  &     1.437  $\pm$     0.159  \\

    Fake l &     1.000  \scriptsize{\it (fixed)}  &     1.000  \scriptsize{\it (fixed)}  &     1.000  \scriptsize{\it (fixed)}  &     1.000  \scriptsize{\it (fixed)}  \\

Combinatoric $D^{*0}$ &     0.888  $\pm$     0.016  &     0.886  $\pm$     0.015  &     1.051  $\pm$     0.043  &     1.039  $\pm$     0.044  \\

   Fake D* &     0.845  $\pm$     0.068  &     0.898  $\pm$     0.061  &     0.841  $\pm$     0.009  &     0.853  $\pm$     0.009  \\

 Continuum &     9.035  \scriptsize{\it (fixed)}  &     9.035  \scriptsize{\it (fixed)}  &     9.035  \scriptsize{\it (fixed)}  &     9.035  \scriptsize{\it (fixed)}  \\
\hline\hline
\end{tabular}


==> tabComparison.tex <==
% Table generated by Excel2LaTeX from sheet 'Summary'
\begin{tabular}{l|@{\extracolsep{.2cm}}cc}
\hline\hline
   & this result & Belle $B^0$ (BN 1054, preliminary)  \\
   \hline
 $\mathcal{F}_1 |V_{cb} | \times 10^3$ &      35.0  $\pm$  0.4  $\pm$   2.2  &      34.4  $\pm$       0.2  $\pm$       1.0  \\
 $\rho^2$ &     1.376  $\pm$     0.074  $\pm$     0.056  &     1.293  $\pm$     0.045  $\pm$     0.029  \\
 $R_1(1)$ &     1.620  $\pm$     0.091  $\pm$     0.092  &     1.495  $\pm$     0.050  $\pm$     0.062  \\
 $R_2(1)$ &     0.805  $\pm$     0.064  $\pm$     0.036  &     0.844  $\pm$     0.034  $\pm$     0.019  \\
\hline\hline

\end{tabular}  

\vspace{.3cm}
    
\begin{tabular}{l|@{\extracolsep{.2cm}}cc}
\hline\hline
   & BaBar $B^0$ \cite{Aubert:2007rs} & Babar $B^+$\cite{Aubert:2007qs} \\
   \hline
$\mathcal{F}_1 |V_{cb} | \times 10^3$ &       34.4  $\pm$   0.3  $\pm$    1.2  &      35.9  $\pm$       0.6  $\pm$       1.4  \\
 $\rho^2$ &     1.191  $\pm$     0.048  $\pm$     0.028  &      1.16  $\pm$      0.06  $\pm$      0.08  \\
 $R_1(1)$ &     1.429  $\pm$     0.061  $\pm$     0.044  &                      -             \\
 $R_2(1)$ &     0.827  $\pm$     0.038  $\pm$     0.022  &                      -             \\
\hline\hline
\end{tabular}
